FedECADO: A Dynamical System Model of Federated Learning

Federated learning harnesses the power of distributed optimization to train a unified machine learning model across separate clients. However, heterogeneous data distributions and computational workloads can lead to inconsistent updates and limit model performance. This work tackles these challenges by proposing FedECADO, a new algorithm inspired by a dynamical system representation of the federated learning process. FedECADO addresses non-IID data distribution through an aggregate sensitivity model that reflects the amount of data processed by each client. To tackle heterogeneous computing, we design a multi-rate integration method with adaptive step-size selections that synchronizes active client updates in continuous time. Compared to prominent techniques, including FedProx and FedNova, FedECADO achieves higher classification accuracies in numerous heterogeneous scenarios.

==> convergence_multirate.tex <==

The multi-rate integration of FedECADO proves to be a key aspect to address heterogeneous computation. In principle, FedECADO identifies that each client simulates its local sub-problem for a different time-window. By linearly interpolation and extrapolating the client updates, FedECADO synchronizes the clients to a global time scale by evaluating the central state at multiple intermediate time-points. In this section, a convergence theorem for FedECADO's multi-rate integration is presented where we demonstrate that each evaluation of the central agent state is a contraction mapping towards an optimum. This derivation employs the analysis for multi-rate waveform relaxation in circuit analysis [XX].


Consider the ODE defined in (XX), that is discretized using a Backward-Euler integration (XX). For the purposes of this convergence analysis, we generalize (XX) to solve for a central agent state, $x_c$, at a time, $t_m$ as:
\begin{equation}
    \rho(x_c) = \Delta t_c \sigma (\nabla f_1 (x_1, I_L^1), \nabla f_2 (x_2, I_L^2), \ldots, \nabla f_n (x_n, I_L^n) ),
\end{equation}

where $\Delta t_c$ is a time-step associated with the central agent. $\rho(\cdot)$ is an operator defined as:
\begin{equation}
    \rho(x_c) = 
\end{equation}
Additionally, $\sigma(\cdot)$ is defined as:
\begin{equation}
    \sigma(\nabla f_1 (x_1, I_L^1), \nabla f_2 (x_2, I_L^2), \ldots, \nabla f_n (x_n, I_L^n)) = 
\end{equation}
Note, we assume that the inverse operation of $\rho(\cdot)$ exists, where:
\begin{equation}
    x_c = \rho^{-1}( \sigma(\nabla f_1 (x_1, I_L^1), \nabla f_2 (x_2, I_L^2), \ldots, \nabla f_n (x_n, I_L^n)))
\end{equation}

Now, as proved in  [XX], it is clear the continuous-time ODE of FedECADO converges to a steady-state where $x_c = x_i \forall t > t_{ss}$ and $I_L^i=0$. We mainly analyze the discretization of the continuous ODE to ensure the Gauss-Jacobi process of solving the entire coupled system converges towards the steady-state (i.e., the local optimum) at each iteration.

The solution process in ECADO (XX) assumes a globally synchronous update, where all client updates are defined at a consistent time-point, $t_m$. Rather, in the federated learning setting, we define an operator, $I_{t_m}\{\cdot\}$, that linearly interpolates and extrapolates the client states to evaluate at a time-point, $t_m$. The operator is defined as:
\begin{equation}
    I_{t} \{ y\} = 
\end{equation}

Due to linearity, two important properties of the operators are:
\begin{itemize}
    \item 
\end{itemize}

\iffalse 
\begin{proof}
In order to analyze the convergence, we represent all the state variables of the central agent, including the central agent state $x_c$ and the flow variables $I_L^i$, as a vector $X=[I_L^1, I_L^2,\ddots, I_L^n, x_c,]$. The ODE for the central agent state in FedECADO, as defined by equations \eqref{eq:multirate_central_ode_be} and \eqref{eq:multirate_central_ode_be_step}, can be generalized as follows: 
\begin{equation} 
\dot{X} = g(X(t), x_i(t)),
\label{eq:general_ode} 
\end{equation} 
where $g(X)$ is defined as
\begin{equation} 
    g(X) = 
    \begin{bmatrix} \sum_{i=1}^n I_L^{i}(\tau_m) \\ x_c^{k+1}(\tau_m) - \Gamma(x_i(t),\tau_m). \end{bmatrix} 
\end{equation} 
Here, $\tau_m$ represents the discretized time point indexed by $m$.
    Furthermore, we generalize the BE integration of the central agent ODE \eqref{eq:central_agent_be_step2} as:
\begin{equation}
    \rho(X^{k+1}(\tau_m)) = \Delta t \sigma( g(X^k(\tau_m), \Gamma(x_1^{k+1}(T_1),\tau_m),\Gamma(x_2^{k+1}(T_1),\tau_m),\cdots )),
\end{equation}
where the operator, $\rho(\cdot)$, is defined as
\begin{equation}
    \rho = \begin{bmatrix}
    1+\frac{\Delta t G_1^{th^{-1}}}{L} & 0 & \ldots & -\frac{\Delta t}{L} \\
         0 & 1+\frac{\Delta t G_2^{th^{-1}}}{L} & \ldots & -\frac{\Delta t}{L}\\
         0 & 0 & \ddots & \frac{-\Delta t}{L} \\
         -\Delta t  & -\Delta t  & \ldots & 1
    \end{bmatrix},
\end{equation}
and $\sigma(\cdot)$, is defined as
\begin{equation}
    \sigma() = \begin{bmatrix}
       -\Gamma(\x_{1}^{k+1}(T_1),\tau_m) + I_1^{k}(\tau_m)G_1^{th^{-1}} \\
       -\Gamma(\x_{2}^{k+1}(T_2),\tau_m) + I_2^{k}(\tau_m)G_2^{th^{-1}} \\
        \vdots \\
        0
    \end{bmatrix}.
\end{equation}
Note, the operator, $\rho(\cdot)$, can be inverted to evaluate the central agent states:
\begin{equation}
    X^{k+1}(\tau) = \Delta t \rho^{-1} \sigma(g(X^k(\tau_m), \Gamma(x_1^{k+1}(T_1),\tau_m),\Gamma(x_2^{k+1}(T_1),\tau_m),\cdots )).
    \label{eq:multirate_proof1}
\end{equation}

The continuous-time ODE of \eqref{eq:multirate_central_ode_be},\eqref{eq:multirate_central_ode_be_step} converges to a stationary point characterized by $x_c = x_i\; \text{for all } i\in C$ and $\dot{I}_L^i=0$. The proof of convergence is provided in [\cite{ecado}]. In this analysis, we study the multi-rate discretization of the ODE to ensure the Gauss-Seidel process of solving the coupled system converges toward the steady state at each iteration. This proof uses the analysis for a multirate waveform relaxation for circuit simulation from [\cite{white2012relaxation}]. This analysis is based on proving that the central agent step is a contraction mapping towards the steady state (i.e., the stationary point of the global objective function).

The multi-rate integration uses the linear operator, $\Gamma(\cdot)$, to interpolate and extrapolate state variables at intermediate time points. Two important properties of the linear operator are the following:
\begin{enumerate}
    \item Given two signals, $y(t)$ and $z(t)$: 
    \begin{equation*}
    \Gamma(y(t)+z(t),\tau) = \Gamma(y(t),\tau) + \Gamma(z(t),\tau) 
    \end{equation*}
    
    \item Given a signal $y(t)$, and a scalar, $\alpha$: 
    \begin{equation*}
        \Gamma(\alpha y(t),\tau) = \alpha \Gamma(y(t),\tau)
    \end{equation*}
    
\end{enumerate}

To prove convergence of the multi-rate integration step, we employ a continuous-time $\beta$ norm defined as:
\begin{equation}
    \|y\|_{\beta} = \text{max}_{[0,T]} e^{-\beta t} [\text{max}_i \Gamma(y_i(t),\tau) \;\; \forall i \in C]
\end{equation}

Under certain conditions, \eqref{eq:multirate_proof1} is a contraction mapping on the $\beta$ norm. To prove this relation, we evaluate the difference between two series, $\{X^k(\tau_m)\}$ and $\{Y^k(\tau_m)\}$, as follows:
\begin{multline}
    \{X^{k+1}(\tau_m)\} - \{Y^{k+1}(\tau_m)\} = \Delta t \rho^{-1}  \sigma(g(X^k(\tau_m), \Gamma(x_1^{k+1}(T_1),\tau_m),\Gamma(x_2^{k+1}(T_1),\tau_m),\cdots )) \\
    - \Delta t \rho^{-1} \sigma(g(Y^k(\tau_m), \Gamma(y_1^{k+1}(T_1),\tau_m),\Gamma(y_2^{k+1}(T_1),\tau_m),\cdots )).
\end{multline}
Exploiting the linearity of the operators, $\Gamma(\cdot)$ and $\rho$, leads to the following:
\begin{multline}
      \{X^{k+1}(\tau_m)\} - \{Y^{k+1}(\tau_m)\} = \Delta t \rho^{-1} \sigma[g(X^k(\tau_m), \Gamma(x_1^{k+1}(T_1),\tau_m),\Gamma(x_2^{k+1}(T_2),\tau_m),\cdots)  \\
      - g(Y^k(\tau_m), \Gamma(y_1^{k+1}(T_1),\tau_m),\Gamma(y_2^{k+1}(T_2),\tau_m),\cdots )].
\end{multline}

The BE operator $\rho^{-1}\sigma(\cdot)$ can be expanded into a series of summations, as shown in Appendix \ref{sec:expanding_be}, using the following equation: 
\begin{multline}
\{X^{k+1}(\tau_m)\} - \{Y^{k+1}(\tau_m)\} = \Delta t \sum_{l=0}^{m} \gamma_l[g(X^k(\tau), \Gamma(x_1^{k+1}(T_1),\tau_{m-l}),\Gamma(x_2^{k+1}(T_1),\tau),\cdots) 
\\ -g(Y^k(\tau), \Gamma(y_1^{k+1}(T_1),\tau),\Gamma(y_2^{k+1}(T_1),\tau),\cdots) ]
\label{eq:multirate_proof_be_operator}
\end{multline} 
where $\gamma_l$ is a scalar that determines the weight of the past state values in the numerical integration method.

To prove that the difference between the series is a contraction mapping, the following two lemmas are useful.

\begin{lemma}
    Given two sequences, \{$X(\tau)$\} and\{$Y(\tau)$\}, if $X(T_i)>Y(T_i)$ $\forall i$, then $\Gamma(X(T_i),\tau) > \Gamma(Y(T_i),\tau)$. Furthermore, if $X(T_i)=K \;\;\forall i$ where $K$ is a constant value, then $\Gamma(X(T_i),\tau)=K$. \label{lm:multirate_lemma1}
\end{lemma}

\begin{lemma}
\label{lm:multirate_lemma2}
    The $\beta$ norm on the following series of $X^K$ is bounded according to the following:
    \begin{equation}
    \label{eq:beta_norm}
        \max_{[0,T]}e^{-\beta \tau} \| \sum_{l=0}^{m}\|\gamma_l \Gamma(X,\tau_{m-l})\|\| \leq \frac{M}{1-e^{-\beta \Delta t}}e^{-\beta \tau} \|\Gamma (X,\tau_m) \|,
    \end{equation}
    where $M$ is equal to $\text{max}_l \| \gamma_l\|$.
\end{lemma}

Proof of the two lemmas is provided in Appendixes \ref{sec:proof_multirate_lemma1} and \ref{sec:proof_multirate_lemma2}. Using Lemma \ref{lm:multirate_lemma1} and the Lipschitz constant of $\nabla f$, we can bound \eqref{eq:multirate_proof_be_operator} as follows:
\begin{equation}
     \{X^{k+1}(\tau)\} - \{Y^{k+1}(\tau)\} \leq  | \sum_{l=0}^{m} |\gamma_l| \left[ \sum_{j=1}^{i}\Delta t_i L_{ij} |\Gamma(X_j^{k+1}-Y_j^{k+1},\tau_{m-l})| + \sum_{j=i+1}^{n}\Delta t_i L_{ij}|\Gamma(X_j^{k}-Y_j^{k},\tau_{m-l})| \right],
\end{equation}
where $L_{ij}$ is the Lipschitz constant of the $i$th row of $g$ with respect to $X_j$. Using the triangle inequality, we formulate this as follows:
\begin{equation}
     \{X^{k+1}(\tau)\} - \{Y^{k+1}(\tau)\} \leq  |  \sum_{j=1}^{i}\Delta t_i L_{ij} \sum_{l=0}^{m} |\gamma_l| |\Gamma(X_j^{k+1}-Y_j^{k+1},\tau_{m-l})| + \sum_{j=i+1}^{n}\Delta t_i L_{ij}\sum_{l=0}^{m} |\gamma_l||\Gamma(X_j^{k}-Y_j^{k},\tau_{m-l})|.
\end{equation}
Multiplying both sides by $e^{-\beta t}$ and taking the maximum over the time window, $[0,T]$, results in the following:
\begin{multline}
     \max_{[0,T]} e^{-\beta t} \{X^{k+1}(\tau)\} - \{Y^{k+1}(\tau)\} \leq  |  \sum_{j=1}^{i}\Delta t_i L_{ij} \max_{[0,T]} e^{-\beta t} \sum_{l=0}^{m} |\gamma_l| |\Gamma(X_j^{k+1}-Y_j^{k+1},\tau_{m-l})| \\ 
     +  \sum_{j=i+1}^{n}\Delta t_i L_{ij} \max_{[0,T]} e^{-\beta t} \sum_{l=0}^{m} |\gamma_l||\Gamma(X_j^{k}-Y_j^{k},\tau_{m-l})|,
\end{multline}
where $T= \text{max}(T_i)$.
Using Lemma \ref{lm:multirate_lemma2}, we conclude the following:
\begin{multline}
     \max_{[0,T]} e^{-\beta t} \{X^{k+1}(\tau)\} - \{Y^{k+1}(\tau)\} \leq \left[\frac{M\Delta t_i}{1-e^{-\beta \Delta t_i}}\sum_{j=1}^{i}L_{ij} \right] \| X^{k+1} - Y^{k+1}\|_\beta \\
     + \left[\frac{M\Delta t_i}{1-e^{-\beta \Delta t_i}}\sum_{j=i+1}^{n}L_{ij} \right] \| X^{k} - Y^{k}\|_\beta ,
\end{multline}
where $\| \cdot\|_\beta$ is the $\beta$ norm defined in \eqref{eq:beta_norm}.

Assuming all time steps, $\Delta t_i>0$ are positive and a $\beta>0$, then there exists a scalar, $\delta>0$ such that:
\begin{equation}
    \delta > \frac{M\Delta t_i}{1-e^{-\beta \Delta t_i}}\sum_{j=i+1}^{n}L_{ij}.
\end{equation}
Using the definition of $\delta$, we conclude the following:
\begin{multline}
     \max_{[0,T]} e^{-\beta t} \{X^{k+1}(\tau)\} - \{Y^{k+1}(\tau)\} \leq \delta \| X^{k+1} - Y^{k+1}\|_\beta      + \delta \| X^{k} - Y^{k}\|_\beta.
\end{multline}
Because the value of $\delta$ holds for all time-steps (indexed by $i$), then:
\begin{multline}
     |\{X^{k+1}(\tau)\} - \{Y^{k+1}(\tau)\}|_\beta \leq \delta \| X^{k+1} - Y^{k+1}\|_\beta      + \delta \| X^{k} - Y^{k}\|_\beta,
\end{multline}
which can be rewritten as:
\begin{equation}
    \| X^{k+1}-Y^{k+1}\|_{\beta} \leq \frac{\delta}{1-\delta} \| X^{k}-Y^{k}\|_{\beta}.
\end{equation}
This proves that for a value of $\delta$ such that $\frac{\delta}{1-\delta}<1$, the multirate integration scheme, $\rho^{-1}\sigma(\cdot)$, is a contraction mapping whereby the series $\{X^{k+1}(\tau)\}$ and $\{Y^{k+1}(\tau)\}$ converges to a stationary point.  


Note, the rate of the contraction mapping, determined by $\frac{\delta}{1-\delta}$, is not affected by the ratio of client step-sizes, $\Delta t_i$. This enables clients to take vastly different step sizes, with accuracy considerations imposed by a Local Truncation Error (LTE). The LTE estimates the error in the approximation of the numerical integration and is a key measure of the accuracy at any iteration.% The LTE for the Backward-Euler integration for the EC model presented in ECADO is derived in [\cite{agarwal2023equivalent}].

To prove convergence to a stationary point of the global objective function, we consider the contraction mapping between two series, $\{X^k\}$ and $\{X^*\}$, where $X^*$ is the state at the stationary point (i.e., $g(X^*)=0$). The difference between the series is diminished according to the contraction mapping:
\begin{equation}
    \|X^{k+1} - X^*\|_{\beta} \leq \frac{\delta}{1-\delta}\|X^{k} - X^*\|_{\beta}.
\end{equation}

This implies that for a $\Delta t$ ensuring $\frac{\delta}{1-\delta}<1$, the FedECADO update asymptotically converges to a stationary point, with a convergence rate determined by $\frac{\delta}{1-\delta}$.
\fi
\end{proof}
